A Comprehensive Comparison of Multi-Dimensional Image Denoising Methods

Filtering multi-dimensional images such as color images, color videos, multispectral images and magnetic resonance images is challenging in terms of both effectiveness and efficiency. Leveraging the nonlocal self-similarity (NLSS) characteristic of images and sparse representation in the transform domain, the block-matching and 3D filtering (BM3D) based methods show powerful denoising performance. Recently, numerous new approaches with different regularization terms, transforms and advanced deep neural network (DNN) architectures are proposed to improve denoising quality. In this paper, we extensively compare over 60 methods on both synthetic and real-world datasets. We also introduce a new color image and video dataset for benchmarking, and our evaluations are performed from four different perspectives including quantitative metrics, visual effects, human ratings and computational cost. Comprehensive experiments demonstrate: (i) the effectiveness and efficiency of the BM3D family for various denoising tasks, (ii) a simple matrix-based algorithm could produce similar results compared with its tensor counterparts, and (iii) several DNN models trained with synthetic Gaussian noise show state-of-the-art performance on real-world color image and video datasets. Despite the progress in recent years, we discuss shortcomings and possible extensions of existing techniques. Datasets and codes for evaluation are made publicly available at https://github.com/ZhaomingKong/Denoising-Comparison.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Table_CC15.tex <==
%% Table generated by Excel2LaTeX from sheet 'Results_all'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Psnr results and average computational time(s) of compared methods on CC15 dataset. The best results are bolded and the second best are underlined.}
%    \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|c|c|}
%    \toprule
%    \multicolumn{2}{|c|}{Methods} & \multicolumn{3}{c|}{CANON 5D ISO = 3200} & \multicolumn{3}{c|}{CANON D600 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 1600} & \multicolumn{3}{c|}{NIKON D800 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 6400} & Average & Time(s) \\
%    \midrule
%    \multicolumn{2}{|c|}{Noisy} & 37.00  & 33.88  & 33.83  & 33.28  & 33.77  & 34.93  & 35.47  & 35.71  & 34.81  & 33.26  & 32.89  & 32.91  & 29.63  & 29.97  & 29.87  & 33.41  & / \\
%    \midrule
%    \multirow{15}[30]{*}{Deep Learning} & TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & 0.63  \\
%\cmidrule{2-19}          & MLP   & 39.01  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & 1.28  \\
%\cmidrule{2-19}          & FFD-Net & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.67  & 1.99  \\
%\cmidrule{2-19}          & CBDNet & 38.63  & 36.18  & 36.10  & 34.83  & 35.69  & 38.32  & 38.44  & 39.98  & 37.29  & 37.78  & 37.15  & 37.39  & 32.58  & 33.01  & 32.01  & 36.36  & 3.58  \\
%\cmidrule{2-19}          & DeepBoosting & 39.74  & 37.23  & 36.87  & 35.39  & 36.98  & 41.08  & 39.72  & 42.02  & 39.68  & 41.42  & 38.76  & 42.34  & 35.78  & 34.48  & 34.27  & 38.38  & 0.32  \\
%\cmidrule{2-19}          & DIDN  & 35.45  & 36.16  & 35.10  & 34.34  & 35.25  & 37.88  & 38.52  & 36.82  & 39.50  & 38.62  & 37.61  & 38.15  & 32.16  & 32.46  & 32.56  & 36.04  & 0.18  \\
%\cmidrule{2-19}          & FCCF  & 41.41  & 37.63  & 37.49  & 36.94  & 39.07  & 42.71  & 39.88  & 42.37  & 40.03  & 41.21  & 38.73  & 41.67  & 36.22  & 35.10  & 35.09  & \textbf{39.04} & 36.36  \\
%\cmidrule{2-19}          & NLNet & 40.57  & 37.05  & 36.86  & 35.26  & 36.80  & 40.47  & 39.03  & 41.53  & 39.19  & 39.37  & 37.13  & 39.83  & 33.68  & 33.33  & 33.26  & 37.56  & 49.98  \\
%\cmidrule{2-19}          & Unet  & 39.72  & 36.75  & 36.54  & 35.28  & 36.53  & 40.47  & 39.09  & 41.13  & 39.33  & 38.50  & 36.89  & 38.75  & 31.69  & 31.88  & 31.74  & 36.95  & 5.69  \\
%\cmidrule{2-19}          & VDNet & 35.68  & 35.32  & 34.93  & 33.73  & 34.92  & 37.55  & 38.27  & 37.23  & 38.56  & 38.19  & 37.69  & 38.54  & 32.45  & 32.26  & 32.65  & 35.86  & 0.21  \\
%\cmidrule{2-19}          & AINDNet & 37.57  & 36.10  & 36.04  & 34.91  & 35.90  & 37.81  & 38.22  & 38.73  & 37.00  & 36.68  & 36.85  & 35.70  & 31.86  & 32.96  & 31.93  & 35.88  & 1.29  \\
%\cmidrule{2-19}          & Noise2Noise & 36.93  & 33.79  & 33.78  & 32.99  & 33.46  & 34.71  & 35.57  & 35.83  & 34.91  & 33.20  & 33.02  & 32.98  & 29.62  & 29.94  & 29.81  & 33.37  & 0.98  \\
%\cmidrule{2-19}          & CycleISP & 36.83  & 35.38  & 35.75  & 34.36  & 35.42  & 37.82  & 38.19  & 39.26  & 37.56  & 35.79  & 35.37  & 35.35  & 31.17  & 31.42  & 31.32  & 35.40  & 0.38  \\
%\cmidrule{2-19}          & SADNet & 38.40  & 37.51  & 36.35  & 35.98  & 37.26  & 41.00  & 39.65  & 41.23  & 39.59  & 39.67  & 37.94  & 41.35  & 33.65  & 34.08  & 33.27  & 37.80  & 0.33  \\
%\cmidrule{2-19}          & DnCNN & 39.51  & 36.92  & 36.54  & 35.02  & 36.46  & 40.59  & 38.94  & 41.33  & 39.05  & 39.57  & 37.43  & 40.18  & 33.56  & 33.53  & 33.41  & 37.47  & 3.28  \\
%    \midrule
%    \midrule
%    \multirow{13}[26]{*}{Traditional Gaussian} & LCSD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 6.45  \\
%\cmidrule{2-19}          & LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>$1000 \\
%\cmidrule{2-19}          & WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.80  & $>$1000 \\
%\cmidrule{2-19}          & GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 38.88  \\
%\cmidrule{2-19}          & MCWNNM & 41.21  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 228.16  \\
%\cmidrule{2-19}          & NLH\_CC & 41.57  & 37.39  & 36.68  & 35.51  & 37.21  & 41.34  & 39.67  & 42.66  & 40.04  & 40.21  & 37.30  & 42.02  & 36.19  & 34.70  & 34.83  & 38.49  & 51.86  \\
%\cmidrule{2-19}          & TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & 37.90  & 368.68  \\
%\cmidrule{2-19}          & CBM3D1 & 40.23  & 37.02  & 36.18  & 34.78  & 36.61  & 40.44  & 38.58  & 41.34  & 39.15  & 39.57  & 37.35  & 39.79  & 34.59  & 33.84  & 33.94  & 37.56  & 0.95  \\
%\cmidrule{2-19}          & CBM3D2 & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.70  & 4.38  \\
%\cmidrule{2-19}          & CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & 37.95  & 4.38  \\
%\cmidrule{2-19}          & M-SVD & 41.43  & 37.17  & 36.84  & 35.20  & 36.97  & 40.23  & 38.90  & 41.75  & 39.60  & 39.33  & 37.26  & 38.70  & 34.52  & 33.53  & 33.74  & 37.68  & 75.88  \\
%\cmidrule{2-19}          & 4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 86.69  \\
%\cmidrule{2-19}          & CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & 37.95  & 6.18  \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:addlabel}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Results_all'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Psnr results and average computational time(s) of compared methods on CC15 dataset. The best results are bolded and the second best are underlined.}
    \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|c|c|}
    \toprule
    \multicolumn{2}{|c|}{Methods} & \multicolumn{3}{c|}{CANON 5D ISO = 3200} & \multicolumn{3}{c|}{CANON D600 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 1600} & \multicolumn{3}{c|}{NIKON D800 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 6400} & Average & Time(s) \\
    \midrule
    \multicolumn{2}{|c|}{Noisy} & 37.00  & 33.88  & 33.83  & 33.28  & 33.77  & 34.93  & 35.47  & 35.71  & 34.81  & 33.26  & 32.89  & 32.91  & 29.63  & 29.97  & 29.87  & 33.41  & / \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{15}[30]{*}{Deep Learning models}} & TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & 0.63  \\
\cmidrule{2-19}          & MLP   & 39.01  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & 1.28  \\
\cmidrule{2-19}          & FFDNet & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.67  & 1.99  \\
\cmidrule{2-19}          & CBDNet & 38.63  & 36.18  & 36.10  & 34.83  & 35.69  & 38.32  & 38.44  & 39.98  & 37.29  & 37.78  & 37.15  & 37.39  & 32.58  & 33.01  & 32.01  & 36.36  & 3.58  \\
\cmidrule{2-19}          & DeepBoosting & 39.74  & 37.23  & 36.87  & 35.39  & 36.98  & 41.08  & 39.72  & 42.02  & 39.68  & 41.42  & 38.76  & 42.34  & 35.78  & 34.48  & 34.27  & 38.38  & 0.32  \\
\cmidrule{2-19}          & DIDN  & 35.45  & 36.16  & 35.10  & 34.34  & 35.25  & 37.88  & 38.52  & 36.82  & 39.50  & 38.62  & 37.61  & 38.15  & 32.16  & 32.46  & 32.56  & 36.04  & 0.18  \\
\cmidrule{2-19}          & FCCF  & 41.41  & 37.63  & 37.49  & 36.94  & 39.07  & 42.71  & 39.88  & 42.37  & 40.03  & 41.21  & 38.73  & 41.67  & 36.22  & 35.10  & 35.09  & \textbf{39.04} & 36.36  \\
\cmidrule{2-19}          & NLNet & 40.57  & 37.05  & 36.86  & 35.26  & 36.80  & 40.47  & 39.03  & 41.53  & 39.19  & 39.37  & 37.13  & 39.83  & 33.68  & 33.33  & 33.26  & 37.56  & 49.98  \\
\cmidrule{2-19}          & Unet  & 39.72  & 36.75  & 36.54  & 35.28  & 36.53  & 40.47  & 39.09  & 41.13  & 39.33  & 38.50  & 36.89  & 38.75  & 31.69  & 31.88  & 31.74  & 36.95  & 5.69  \\
\cmidrule{2-19}          & VDNet & 35.68  & 35.32  & 34.93  & 33.73  & 34.92  & 37.55  & 38.27  & 37.23  & 38.56  & 38.19  & 37.69  & 38.54  & 32.45  & 32.26  & 32.65  & 35.86  & 0.21  \\
\cmidrule{2-19}          & AINDNet & 37.57  & 36.10  & 36.04  & 34.91  & 35.90  & 37.81  & 38.22  & 38.73  & 37.00  & 36.68  & 36.85  & 35.70  & 31.86  & 32.96  & 31.93  & 35.88  & 1.29  \\
\cmidrule{2-19}          & Noise2Noise & 36.93  & 33.79  & 33.78  & 32.99  & 33.46  & 34.71  & 35.57  & 35.83  & 34.91  & 33.20  & 33.02  & 32.98  & 29.62  & 29.94  & 29.81  & 33.37  & 0.98  \\
\cmidrule{2-19}          & CycleISP & 36.83  & 35.38  & 35.75  & 34.36  & 35.42  & 37.82  & 38.19  & 39.26  & 37.56  & 35.79  & 35.37  & 35.35  & 31.17  & 31.42  & 31.32  & 35.40  & 0.38  \\
\cmidrule{2-19}          & SADNet & 38.40  & 37.51  & 36.35  & 35.98  & 37.26  & 41.00  & 39.65  & 41.23  & 39.59  & 39.67  & 37.94  & 41.35  & 33.65  & 34.08  & 33.27  & 37.80  & 0.33  \\
\cmidrule{2-19}          & DnCNN & 39.51  & 36.92  & 36.54  & 35.02  & 36.46  & 40.59  & 38.94  & 41.33  & 39.05  & 39.57  & 37.43  & 40.18  & 33.56  & 33.53  & 33.41  & 37.47  & 3.28  \\
    \midrule
    \midrule
    \multicolumn{1}{|c|}{\multirow{13}[26]{*}{Traditional Gaussian Denoiser}} & LCSD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 6.45  \\
\cmidrule{2-19}          & LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>$1000 \\
\cmidrule{2-19}          & WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.80  & $>$2000 \\
\cmidrule{2-19}          & GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 38.88  \\
\cmidrule{2-19}          & MCWNNM & 41.21  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 228.16  \\
\cmidrule{2-19}          & NLH\_CC & 41.57  & 37.39  & 36.68  & 35.51  & 37.21  & 41.34  & 39.67  & 42.66  & 40.04  & 40.21  & 37.30  & 42.02  & 36.19  & 34.70  & 34.83  & 38.49  & 51.86  \\
\cmidrule{2-19}          & TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & 37.90  & 368.68  \\
\cmidrule{2-19}          & CBM3D1 & 40.23  & 37.02  & 36.18  & 34.78  & 36.61  & 40.44  & 38.58  & 41.34  & 39.15  & 39.57  & 37.35  & 39.79  & 34.59  & 33.84  & 33.94  & 37.56  & 0.95  \\
\cmidrule{2-19}          & CBM3D2 & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.70  & 4.38  \\
\cmidrule{2-19}          & CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & 37.95  & 4.38  \\
\cmidrule{2-19}          & M-SVD & 41.43  & 37.17  & 36.84  & 35.20  & 36.97  & 40.23  & 38.90  & 41.75  & 39.60  & 39.33  & 37.26  & 38.70  & 34.52  & 33.53  & 33.74  & 37.68  & 75.88  \\
\cmidrule{2-19}          & 4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 86.69  \\
\cmidrule{2-19}          & CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & 37.95  & 6.18  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Table_Color_other_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'Results_all'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Psnr results of compared methods on CC60, Xu-100 and Kong-Image dataset. The three best results are bolded.}
    \begin{tabular}{c|cccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{11}{c}{Dataset} \\
\cmidrule{3-13}    \multicolumn{2}{c}{} & CC60  & Xu-100 & CANON 100D & CANON 600D & HUAWEI & IPHONE 5S & IPHONE 6S & SONY & XIAOMI & OPPO & FUJIFILM \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  \\
    \midrule
    \multirow{12}[24]{*}{Deep Learning Models} & FFD-Net & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  \\
\cmidrule{2-13}          & CBDNet & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  \\
\cmidrule{2-13}          & DeepBoosting & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  \\
\cmidrule{2-13}          & DIDN  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  \\
\cmidrule{2-13}          & FCCF  & 40.89  & 38.85 & 41.91  & 43.07  & 40.11  & 40.39  & 40.65  & 45.38  & 36.67  & 40.93  & 42.78  \\
\cmidrule{2-13}          & NLNet & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  \\
\cmidrule{2-13}          & Unet  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  \\
\cmidrule{2-13}          & VDNet & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  \\
\cmidrule{2-13}          & AINDNet & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  \\
\cmidrule{2-13}          & CycleISP & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  \\
\cmidrule{2-13}          & SADNet & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  \\
\cmidrule{2-13}          & DnCNN & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{\multirow{11}[22]{*}{Traditional Gaussian Denoisers}} & LCSD  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  \\
\cmidrule{2-13}          & LLRT  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  \\
\cmidrule{2-13}          & GID   & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  \\
\cmidrule{2-13}          & MCWNNM & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  \\
\cmidrule{2-13}          & NLH\_CC & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  \\
\cmidrule{2-13}          & TWSC  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  \\
\cmidrule{2-13}          & CBM3D1 & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  \\
\cmidrule{2-13}          & CBM3D2 & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  \\
\cmidrule{2-13}          & CBM3D\_best & 39.68 & 38.81 & 42.08 & 42.89 & 40.48 & 41.25 & 41.16 & 45.81 & 36.66  & 40.89  & 43.14  \\
\cmidrule{2-13}          & 4DHOSVD1 & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  \\
\cmidrule{2-13}          & CMSt-SVD & 39.75 & 38.82 & 41.99  & 42.75  & 40.08  & 40.84  & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Table_Method_all.tex <==
%\begin{table*}
%\scriptsize
%\centering
%\caption{aa}
%\scalebox{0.88}{
%\renewcommand{\arraystretch}{1.02}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%Category                      & Representation           & Methods       & Noise Modeling Experiments      & Applications     & Key Words                                                     \\
%\hline
%\multirow{41}{*}{Traditional} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color, othman2006noise}           & AWGN                            & CI, MSI          & Adaptive wavelet thresholding with thresholding techniques    \\
%\cline{3-6}
%                              &                          & NLM \cite{buades2005review, dai2013multichannel}          & AWGN                            & CI               & NLM algorithm with Gaussian kernels                           \\
%\cline{3-6}
%                              &                          & WSM \cite{coupe20083d}          & AWGN                            & MRI              & 3D wavelet subbands mixing for image denoising                \\
%\cline{3-6}
%                              &                          & TCVD \cite{liu2010high}         & AWGN                            & CV               & Integration of robust optical flow into NLM                   \\
%\cline{3-6}
%                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                            & CI, MRI          & Applications of SVD decomposition                             \\
%\cline{3-6}
%                              &                          & LRMR \cite{zhang2013hyperspectral}          & AWGN                            & MRI              & A low-rank matrix decomposition model                         \\
%\cline{3-6}
%                              &                          & GID \cite{xu2018external}          & AWGN                            & CI               & External data guided and internal prior learning              \\
%\cline{3-6}
%                              &                          & SPTWO \cite{buades2016patch}        & AWGN                            & CV               & NLPCA with optical flow estimation                            \\
%\cline{3-6}
%                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                            & CI, MSI          & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                            & CV               & Efficient approximate global patch search                     \\
%\cline{3-6}
%                              &                          & MCWNNM \cite{xu2017multi}       & AWGN                            & CI               & Extension of WNNM to color images                             \\
%\cline{3-6}
%                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                            & CV               & ~A trilateral weighted sparse coding scheme                   \\
%\cline{3-6}
%                              &                          & NLH\_CC \cite{hou2020nlh}      & AWGN                            & CI               & Nonlocal pixel similarity with Haar transform                 \\
%\cline{3-6}
%                              &                          & AMF \cite{chan2005salt}          & Impulsive                       & CI               & Impulsive noise removal by adaptive median filter             \\
%\cline{3-6}
%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                       & CI               & Impulsive noise removal by iterative adaptive fuzzy filter    \\
%\cline{3-6}
%                              &                          & LSM-NLR \cite{huang2017mixed}      & Gaussian, Poisson and Impulsive & CV               & Low-rank with laplacian scale mixture modeling                \\
%\cline{3-6}
%                              &                          & FastHyde \cite{zhuang2018fast}     & Gaussian and Poisson        & MSI              & Low-rank and sparse representation                            \\
%\cline{3-6}
%                              &                          & NMoG \cite{chen2017denoising}         & Gaussian, Stripe and Impulsive  & MSI              & Low-rank matrix model with non i.i.d Gaussian noise           \\
%\cline{3-6}
%                              &                          & ODCT \cite{manjon2012new}         & AWGN and Rician                 & MRI              & A 3D DCT implementation                                       \\
%\cline{3-6}
%                              &                          & OBNLM \cite{coupe2008optimized}        & AWGN and Rician                 & MRI              & An optimized blockwise NLM Filter                             \\
%\cline{3-6}
%                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician                 & MRI              & Adaptive NLM with spatially varying noise levels              \\
%\cline{3-6}
%                              &                          & RLMMSE \cite{aja2008noise}       & Rician                          & MRI              & A novel linear minimum mean square error (LMMSE) estimator    \\
%\cline{3-6}
%                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician                 & MRI              & A rotationally invariant version of the NLM filter            \\
%\cline{3-6}
%                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician                 & MRI              & A two stage filter based on NLPCA and PRI-NLM                 \\
%\cline{2-6}
%                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                            & CI               & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}       & AWGN                            & CV               & Extention of CBM3D to color videos                            \\
%\cline{3-6}
%                              &                          & LRTA \cite{renard2008denoising}         & AWGN                            & MSI              & A low Tucker rank tensor decomposition  model                 \\
%\cline{3-6}
%                              &                          & PARAFAC \cite{liu2012denoising}      & AWGN                            & MSI              & A rank-one CP decomposition model                             \\
%\cline{3-6}
%                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                            & CV               & Extention of BM3D to color videos using 3D patch              \\
%\cline{3-6}
%                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                            & MSI, MRI         & Extention of BM4D to MSI and MRI using 3D patch               \\
%\cline{3-6}
%                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising}      & AWGN                            & CI, MSI, MRI     & Applications of 4DHOSVD transform                             \\
%\cline{3-6}
%                              &                          & TDL \cite{peng2014decomposable}           & AWGN                            & MSI              & A Tucker based tensor dictionary learning algorithm           \\
%\cline{3-6}
%                              &                          & KTSVD \cite{Zhang2015KTSVD}        & AWGN                            & MSI              & A t-SVD based tensor dictionary learning algorithm            \\
%\cline{3-6}
%                              &                          & ITSReg \cite{xie2016multispectral}       & AWGN                            & MSI              & Intrinsic Tensor Sparsity Regularization                      \\
%\cline{3-6}
%                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                            & MSI              & Low Tucker rank decomposition with total variation            \\
%\cline{3-6}
%                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                            & CI               & A weighted rank-one CP decomposition model                    \\
%\cline{3-6}
%                              &                          & HOSVDR\_S \cite{lv2019denoising}    & AWGN                            & MRI              & A recursive low Tucker rank model with rank estimation        \\
%\cline{3-6}
%                              &                          & MSt-SVD \cite{kong2017new, kong2019color}      & AWGN                            & CI, CV, MRI, MSI & An efficient one-stage multi-diemsional t-SVD implementation  \\
%\cline{3-6}
%                              &                          & NGMeet \cite{he2019non}        & AWGN                            & MSI              & Low-rank tensor model with iterative regularization           \\
%\cline{3-6}
%                              &                          & LTDL \cite{gong2020low}         & AWGN                            & MSI              & A low-rank tensor dictionary learning method                  \\
%\cline{3-6}
%                              &                          & NLTA-LSM \cite{dong2015low}     & Gaussian and Poisson         & MSI, MRI         & Low Tucker rank with laplacian scale mixture modeling         \\
%\hline
%\end{tabular}
%}
%\end{table*}

% \usepackage{multirow}

\begin{table*}[htbp]
\scriptsize
\centering
\caption{Related multi-dimensional image denoising methods with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'MRI': magnetic resonance imaging.}
\scalebox{0.84}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
\hline
\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding with thresholding techniques    \\
\cline{3-6}
                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & high-quality denoising with discrete cosine transform (DCT)   \\
\cline{3-6}
                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & NLM algorithm with Gaussian kernels                           \\
\cline{3-6}
                              &                          & WSM \cite{coupe20083d}           & AWGN                        & MRI               & 3D wavelet subbands mixing for image denoising                \\
\cline{3-6}
                              &                          & K-SVD \cite{mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & 3D wavelet over-complete dictionary learning and sparse coding                \\
\cline{3-6}
                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Integration of robust optical flow into NLM                   \\
\cline{3-6}
                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD decomposition                             \\
\cline{3-6}
                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian patch-based method for whole image restoration                          \\
\cline{3-6}
                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
\cline{3-6}
                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
\cline{3-6}
                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
\cline{3-6}
                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
\cline{3-6}
                              &                          & MCWNNM \cite{xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
\cline{3-6}
                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
\cline{3-6}
                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
\cline{3-6}
                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
\cline{3-6}
                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
\cline{3-6}
                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
\cline{3-6}
                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
\cline{3-6}
                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
\cline{3-6}
                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
\cline{3-6}
                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
\cline{3-6}
                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
\cline{3-6}
                              &                          & OBNLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
\cline{3-6}
                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
\cline{3-6}
                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error (LMMSE) estimator    \\
\cline{3-6}
                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
\cline{3-6}
                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
\cline{2-6}
                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
\cline{3-6}
                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
\cline{3-6}
                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one CP decomposition model                             \\
\cline{3-6}
                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
\cline{3-6}
                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM4D to MSI and MRI using 3D patch               \\
\cline{3-6}
                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
\cline{3-6}
                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
\cline{3-6}
                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
\cline{3-6}
                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
\cline{3-6}
                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
\cline{3-6}
                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
\cline{3-6}
                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
\cline{3-6}
                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
\cline{3-6}
                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
\cline{3-6}
                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-stage t-SVD implementation  \\
\cline{3-6}
                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
\cline{3-6}
                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
\cline{3-6}
                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
\hline
\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
\hline
\multirow{32}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{22}{*}{CNN}    & DnCNN \cite{zhang2017beyond, jiang2018denoising}       & AWGN                        & CI, MRI           & Residual learning and batch normalization                     \\
\cline{3-6}
                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
\cline{3-6}
                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
\cline{3-6}
                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
\cline{3-6}
                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
\cline{3-6}
                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
\cline{3-6}
                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
\cline{3-6}
                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
\cline{3-6}
                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
\cline{3-6}
                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & A real-time method without flow estimation                    \\
\cline{3-6}
                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
\cline{3-6}
                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
\cline{3-6}
                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
\cline{3-6}
                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
\cline{3-6}
                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
\cline{3-6}
                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
\cline{3-6}
                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
\cline{3-6}
                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
\cline{3-6}
                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
\cline{3-6}
                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering and CNN                     \\
\cline{3-6}
                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
\cline{3-6}
                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
\cline{3-6}
                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
\cline{3-6}
                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
\cline{3-6}
                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
\cline{3-6}
                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
\cline{2-6}
                              & \multirow{10}{*}{Others} & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\
\cline{3-6}
                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
\cline{3-6}
                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
\cline{3-6}
                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
%\cline{3-6}
%                              &                          & LLRefineNet \cite{jiang2018deep}  & AWGN and Impulsive          & CI                & Encoder-decoder network with skip connections                 \\
\cline{3-6}
                              &                          & GCBD \cite{Chen_2018_CVPR}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
\cline{3-6}
                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
\cline{3-6}
                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
\cline{3-6}
                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
\cline{3-6}
                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
\cline{3-6}
                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
\cline{3-6}
                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
\hline
\end{tabular}
}
\label{Table_Method_all}
\end{table*}



==> Table_Method_all_new.tex <==
\begin{table*}[htbp]
\scriptsize
\centering
\caption{Related multi-dimensional image denoising methods with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'HSI': hyperspectral imaging, 'MRI': magnetic resonance imaging.}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
\hline
\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding with thresholding techniques    \\
\cline{3-6}
                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & high-quality denoising with discrete cosine transform (DCT)   \\
\cline{3-6}
                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & NLM algorithm with Gaussian kernels                           \\
\cline{3-6}
                              &                          & K-SVD \cite{mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & 3D wavelet over-complete dictionary learning and sparse coding                \\
\cline{3-6}
                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Combination of robust optical flow with NLM                   \\
\cline{3-6}
                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD decomposition                             \\
\cline{3-6}
                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian patch-based method for whole image restoration                          \\
\cline{3-6}
                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
\cline{3-6}
                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
\cline{3-6}
                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
\cline{3-6}
                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
\cline{3-6}
                              &                          & MCWNNM \cite{xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
\cline{3-6}
                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
\cline{3-6}
                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
\cline{3-6}
                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
\cline{3-6}
                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
%\cline{3-6}
%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
\cline{3-6}
                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
\cline{3-6}
                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
\cline{3-6}
                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
\cline{3-6}
                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
\cline{3-6}
                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
\cline{3-6}
                              &                          & OBNLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
\cline{3-6}
                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
\cline{3-6}
                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error (LMMSE) estimator    \\
\cline{3-6}
                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
\cline{3-6}
                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
\cline{2-6}
                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
\cline{3-6}
                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
\cline{3-6}
                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one CP decomposition model                             \\
\cline{3-6}
                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
\cline{3-6}
                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM4D to MSI and MRI using 3D patch               \\
\cline{3-6}
                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
\cline{3-6}
                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
\cline{3-6}
                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
\cline{3-6}
                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
\cline{3-6}
                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
\cline{3-6}
                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
\cline{3-6}
                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
\cline{3-6}
                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
\cline{3-6}
                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
\cline{3-6}
                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-stage t-SVD implementation  \\
\cline{3-6}
                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
\cline{3-6}
                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
\cline{3-6}
                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
\hline
\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
\hline
\multirow{32}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{29}{*}{CNN/NN}   & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\

\cline{3-6}
                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
\cline{3-6}
                              &                          & DnCNN \cite{zhang2017beyond, jiang2018denoising}          & AWGN                        & CI, MRI                 & CNN with Residual learning and batch normalization                       \\
\cline{3-6}
                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
\cline{3-6}
                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
\cline{3-6}
                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
\cline{3-6}
                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
\cline{3-6}
                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
\cline{3-6}
                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
\cline{3-6}
                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
\cline{3-6}
                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
\cline{3-6}
                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & A real-time method without flow estimation                    \\
\cline{3-6}
                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
\cline{3-6}
                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
\cline{3-6}
                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
\cline{3-6}
                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
\cline{3-6}
                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
\cline{3-6}
                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
\cline{3-6}
                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
\cline{3-6}
                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
\cline{3-6}
                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
\cline{3-6}
                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
\cline{3-6}
                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
\cline{3-6}
                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering and CNN                     \\
\cline{3-6}
                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
\cline{3-6}
                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
\cline{3-6}
                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
\cline{3-6}
                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
\cline{3-6}
                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
\cline{3-6}
                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
\cline{2-6}
                              & \multirow{8}{*}{CNN + GAN} & GCBD \cite{Chen_2018_CVPR}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
\cline{3-6}
                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
\cline{3-6}
                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
\cline{3-6}
                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
\cline{3-6}
                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
\cline{3-6}
                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
\cline{3-6}
                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
\hline
\end{tabular}
}
\label{Table_Method_all}
\end{table*}



==> Table_color_all_psnr.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\renewcommand{\arraystretch}{0.9}
%\tiny
%  \centering
%  \caption{Average PSNR and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$.}
%  \scalebox{0.96}{
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset}                                                                  & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
%\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI &       &  \\
%    \midrule
%    \multicolumn{2}{c}{Noisy} & 33.41 & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & MATLAB + MEX & 1.99  \\
%    \midrule
%    \multirow{12}[24]{*}{Deep Network} & FFDNet & 37.67  & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & MATLAB + MEX & 3.58  \\
%\cmidrule{2-16}          & CBDNet & 36.36  & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & Python + GPU & 0.32  \\
%\cmidrule{2-16}          & DeepBoosting & 38.38  & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & Python + GPU & 0.18  \\
%\cmidrule{2-16}          & DIDN  & 36.04  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & Python + GPU & 0.98  \\
%\cmidrule{2-16}          & FCCF  & 39.04  & 40.89  & 38.85 & 41.91  & 43.07  & 40.11  & 40.39  & 40.65  & 45.38  & 36.67  & 40.93  & 42.78  & MATLAB + MEX & 49.98  \\
%\cmidrule{2-16}          & NLNet & 37.56  & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & MATLAB + MEX & 5.69  \\
%\cmidrule{2-16}          & Unet  & 36.95  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & Python + GPU & 0.21  \\
%\cmidrule{2-16}          & VDNet & 35.86  & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & Python + GPU & 1.29  \\
%\cmidrule{2-16}          & AINDNet & 35.88  & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & Python + GPU & 0.98  \\
%\cmidrule{2-16}          & CycleISP & 35.40  & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & Python + GPU & 0.38  \\
%\cmidrule{2-16}          & SADNet & 37.80  & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & Python + GPU & 0.33  \\
%\cmidrule{2-16}          & DnCNN & 37.47  & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & MATLAB + MEX & 3.28  \\
%    \midrule
%    \midrule
%    \multirow{12}[24]{*}{Gaussian} & LCSD  & 36.20  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & MATLAB + MEX & 6.45  \\
%\cmidrule{2-16}          & LLRT  & 37.36  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & Pure MATLAB & $>$1000 \\
%\cmidrule{2-16}          & GID   & 37.02  & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & Pure MATLAB  & 38.88  \\
%\cmidrule{2-16}          & MCWNNM & 37.72  & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & Pure MATLAB & 228.16  \\
%\cmidrule{2-16}          & NLH\_CC & 38.49  & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  & MATLAB + MEX & 51.86  \\
%\cmidrule{2-16}          & TWSC  & 37.90  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & Pure MATLAB & 368.68  \\
%\cmidrule{2-16}          & CBM3D1 & 37.56  & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & MATLAB + MEX & 0.95  \\
%\cmidrule{2-16}          & CBM3D2 & 37.70  & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & MATLAB + MEX & 4.38  \\
%\cmidrule{2-16}          & M-SVD & 37.62  & 39.27 & 38.56 & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & Pure MATLAB & 4.38  \\
%\cmidrule{2-16}          & CBM3D\_best & 37.95  & 39.68 & 38.81 & 42.08 & 42.89 & 40.48 & 41.25 & 41.16 & 45.81 & 36.66  & 40.89  & 43.14  & Pure MATLAB & 75.88  \\
%\cmidrule{2-16}          & 4DHOSVD1 & 37.51  & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & Pure MATLAB & 86.69  \\
%\cmidrule{2-16}          & CMSt-SVD & 37.95  & 39.75 & 38.82 & 41.99  & 42.75  & 40.08  & 40.84  & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  & MATLAB + MEX & 6.18  \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_color_all_psnr}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR values and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$. The best results are black bolded.}
    \scalebox{0.96}{
    \renewcommand{\arraystretch}{0.69}
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset}                                                                  & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO& FUJIFILM &       &  \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 33.41 & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & MATLAB + MEX & 1.99  \\
    \midrule
    \multirow{12}[24]{*}{\shortstack[l]{Deep \\ Network}} & FFDNet & 37.67  & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & MATLAB + MEX & 3.58  \\
\cmidrule{2-16}          & CBDNet & 36.36  & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & Python + GPU & 0.32  \\
\cmidrule{2-16}          & DeepBoosting & 38.38  & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & Python + GPU & 0.18  \\
\cmidrule{2-16}          & DIDN  & 36.04  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & Python + GPU & 0.98  \\
\cmidrule{2-16}          & FCCF  & \textbf{39.04} & \textbf{40.89} & \textbf{38.85} & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.67} & \textbf{40.93} & 42.78  & MATLAB + MEX & 49.98  \\
\cmidrule{2-16}          & NLNet & 37.56  & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & MATLAB + MEX & 5.69  \\
\cmidrule{2-16}          & Unet  & 36.95  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & Python + GPU & 0.21  \\
\cmidrule{2-16}          & VDNet & 35.86  & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & Python + GPU & 1.29  \\
\cmidrule{2-16}          & AINDNet & 35.88  & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & Python + GPU & 0.98  \\
\cmidrule{2-16}          & CycleISP & 35.40  & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & Python + GPU & 0.38  \\
\cmidrule{2-16}          & SADNet & 37.80  & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & Python + GPU & 0.33  \\
\cmidrule{2-16}          & DnCNN & 37.47  & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & MATLAB + MEX & 3.28  \\
    \midrule
    \midrule
    \multirow{12}[24]{*}{\shortstack[l]{Traditional \\ Denoiser}} & LSCD  & 36.20  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & MATLAB + MEX & 6.45  \\
\cmidrule{2-16}          & LLRT  & 37.36  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & Pure MATLAB & $>$1000 \\
\cmidrule{2-16}          & GID   & 37.02  & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & Pure MATLAB & 38.88  \\
\cmidrule{2-16}          & MCWNNM & 37.72  & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & Pure MATLAB & 228.16  \\
\cmidrule{2-16}          & NLH\_CC & 38.49  & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00 } & 35.73  & 40.69  & 42.80  & MATLAB + MEX & 51.86  \\
\cmidrule{2-16}          & TWSC  & 37.90  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & Pure MATLAB & 368.68  \\
\cmidrule{2-16}          & CBM3D1 & 37.56  & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & MATLAB + MEX & 0.95  \\
\cmidrule{2-16}          & CBM3D2 & 37.70  & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & MATLAB + MEX & 4.38  \\
\cmidrule{2-16}          & M-SVD & 37.62  & 39.27 & 38.56 & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & Pure MATLAB & 4.38  \\
\cmidrule{2-16}          & CBM3D\_best & 37.95  & 39.68 & \textbf{38.81} & \textbf{42.08} & 42.89 & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & \textbf{45.81} & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & MATLAB + mex & 75.88  \\
\cmidrule{2-16}          & 4DHOSVD1 & 37.51  & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & Pure MATLAB & 86.69  \\
\cmidrule{2-16}          & CMSt-SVD & 37.95  & 39.75 & \textbf{38.82} & \textbf{41.99} & 42.75  & 40.08  & 40.84  & 40.53  & \textbf{45.89} & 36.40  & \textbf{40.85} & 42.68  & MATLAB + MEX & 6.18  \\
    \bottomrule
    \end{tabular}}%
  \label{Table_color_all_psnr}%
\end{table*}%



==> Table_color_all_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{c|ccccccccccccc}
%    \multicolumn{2}{c}{\multirow{2}[3]{*}{Method}} & \multicolumn{12}{c}{Dataset} \\
%\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI \\
%    \midrule
%    \multicolumn{2}{c}{Noisy} & 0.8476 & 0.8712 & 0.9125 & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251 & 0.9356  & 0.9307  \\
%    \midrule
%    \multirow{12}[24]{*}{Deep Network} & FFD-Net & 0.9563 & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  \\
%\cmidrule{2-14}          & CBDNet & 0.9294 & 0.9482 & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  \\
%\cmidrule{2-14}          & DeepBoosting & 0.9644 & 0.9811 & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  \\
%\cmidrule{2-14}          & DIDN  & 0.9456 & N/A   & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  \\
%\cmidrule{2-14}          & FCCF  & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852 } & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640 } & \textbf{0.9747 } & 0.9782  \\
%\cmidrule{2-14}          & NLNet & 0.9554 & 0.9744 & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  \\
%\cmidrule{2-14}          & Unet  & 0.9425 & 0.9708 & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  \\
%\cmidrule{2-14}          & VDNet & 0.9454 & N/A   & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  \\
%\cmidrule{2-14}          & AINDNet & 0.9113 & 0.9708 & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  \\
%\cmidrule{2-14}          & CycleISP & 0.9158 & 0.9393 & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  \\
%\cmidrule{2-14}          & SADNet & 0.9521 & N/A   & 0.9725  & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  \\
%\cmidrule{2-14}          & DnCNN & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  \\
%    \midrule
%    \midrule
%    \multirow{12}[24]{*}{Gaussian Denoiser} & LCSD  & 0.9339 & 0.9626 & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  \\
%\cmidrule{2-14}          & LLRT  & 0.9559 & 0.9636 & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  \\
%\cmidrule{2-14}          & GID   & 0.9459 & 0.9633 & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  \\
%\cmidrule{2-14}          & MCWNNM & 0.9568 & 0.9698 & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  \\
%\cmidrule{2-14}          & NLH\_CC & 0.9647 & 0.9759 & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905 } & 0.9552  & 0.9740  & 0.9776  \\
%\cmidrule{2-14}          & TWSC  & 0.9592 & 0.9759 & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  \\
%\cmidrule{2-14}          & CBM3D1 & 0.9562 & 0.9729 & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  \\
%\cmidrule{2-14}          & CBM3D2 & 0.9572 & 0.974 & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  \\
%\cmidrule{2-14}          & M-SVD & 0.9542 & 0.9705 & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  \\
%\cmidrule{2-14}          & CBM3D\_best & 0.9621 & 0.9775 & \textbf{0.9712 } & \textbf{0.9808 } & \textbf{0.9851 } & \textbf{0.9741 } & \textbf{0.9758 } & \textbf{0.9783 } & \textbf{0.9904 } & \textbf{0.9640 } & 0.9742  & \textbf{0.9805 } \\
%\cmidrule{2-14}          & 4DHOSVD1 & 0.9559 & 0.9729 & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  \\
%\cmidrule{2-14}          & CMSt-SVD & 0.9588 & 0.9756 & 0.9694  & 0.9794  & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903 } & 0.9616  & \textbf{0.9743 } & 0.9770  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_color_all_ssim}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\tiny
  \centering
    \caption{Average SSIM values of compared methods on CC15, Xu-100 and Kong-Image datasets. The best results are black bolded.}
    \renewcommand{\arraystretch}{0.69}
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset} \\
\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 0.8476 & 0.8712 & 0.9125 & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251 & 0.9356  & 0.9307  \\
    \midrule
    \multirow{12}[24]{*}{Deep Network} & FFDNet & 0.9563 & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  \\
\cmidrule{2-14}          & CBDNet & 0.9294 & 0.9482 & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  \\
\cmidrule{2-14}          & DeepBoosting & 0.9644 & 0.9811 & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  \\
\cmidrule{2-14}          & DIDN  & 0.9456 & N/A   & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  \\
\cmidrule{2-14}          & FCCF  & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & 0.9782  \\
\cmidrule{2-14}          & NLNet & 0.9554 & 0.9744 & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  \\
\cmidrule{2-14}          & Unet  & 0.9425 & 0.9708 & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  \\
\cmidrule{2-14}          & VDNet & 0.9454 & N/A   & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  \\
\cmidrule{2-14}          & AINDNet & 0.9113 & 0.9708 & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  \\
\cmidrule{2-14}          & CycleISP & 0.9158 & 0.9393 & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  \\
\cmidrule{2-14}          & SADNet & 0.9521 & N/A   & 0.9725  & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  \\
\cmidrule{2-14}          & DnCNN & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  \\
    \midrule
    \midrule
    \multirow{12}[24]{*}{Gaussian Denoiser} & LSCD  & 0.9339 & 0.9626 & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  \\
\cmidrule{2-14}          & LLRT  & 0.9559 & 0.9636 & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  \\
\cmidrule{2-14}          & GID   & 0.9459 & 0.9633 & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  \\
\cmidrule{2-14}          & MCWNNM & 0.9568 & 0.9698 & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  \\
\cmidrule{2-14}          & NLH\_CC & 0.9647 & 0.9759 & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905} & 0.9552  & 0.9740  & 0.9776  \\
\cmidrule{2-14}          & TWSC  & 0.9592 & 0.9759 & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  \\
\cmidrule{2-14}          & CBM3D1 & 0.9562 & 0.9729 & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  \\
\cmidrule{2-14}          & CBM3D2 & 0.9572 & 0.974 & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  \\
\cmidrule{2-14}          & M-SVD & 0.9542 & 0.9705 & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  \\
\cmidrule{2-14}          & CBM3D\_best & 0.9621 & 0.9775 & \textbf{0.9712} & \textbf{0.9808} & \textbf{0.9851} & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & \textbf{0.9904} & \textbf{0.9640} & 0.9742  & \textbf{0.9805} \\
\cmidrule{2-14}          & 4DHOSVD1 & 0.9559 & 0.9729 & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  \\
\cmidrule{2-14}          & CMSt-SVD & 0.9588 & 0.9756 & 0.9694  & 0.9794  & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903} & 0.9616  & \textbf{0.9743} & 0.9770  \\
    \bottomrule
    \end{tabular}%
  \label{Table_color_all_ssim}%
\end{table*}%

